EdgeRec: Recommender System on Edge in Mobile Taobao

Recommender system (RS) has become a crucial module in most web-scale applications. Recently, most RSs are in the waterfall form based on the cloud-to-edge framework, where recommended results are transmitted to edge (e.g., user mobile) by computing in advance in the cloud server. Despite effectiveness, network bandwidth and latency between cloud server and edge may cause the delay for system feedback and user perception. Hence, real-time computing on edge could help capture user preferences more preciously and thus make more satisfactory recommendations. Our work, to our best knowledge, is the first attempt to design and implement the novel Recommender System on Edge (EdgeRec), which achieves Real-time User Perception and Real-time System Feedback. Moreover, we propose Heterogeneous User Behavior Sequence Modeling and Context-aware Reranking with Behavior Attention Networks to capture user's diverse interests and adjust recommendation results accordingly. Experimental results on both the offline evaluation and online performance in Taobao home-page feeds demonstrate the effectiveness of EdgeRec.

==> implementation.tex <==
\section{System Implementation and Deployment}
\label{sec:implementation}

==> related.tex <==
\section{Industrial Recommender Systems}
%\label{sec:related}
%\subsection{Industrial Recommender Systems}
\label{sec:rs_related}
Industrial RS usually consists of the matching stage and ranking stage (see Fig. \ref{fig:motivation}),
in order to handle the billion-scale of users and items~\cite{covington2016deep}.
The matching stage~\cite{li2019multi,zhu2018learning} is responsible for
retrieving thousands of candidate items that are relevant to user interests.
In the ranking stage, we first predict click-through-rate (CTR)~\cite{zhou2018deep,zhou2019deep} and conversion-rate (CVR)~\cite{ma2018entire}
of users interacting with these candidate items (e.g., click or buy).
And then apply learning-to-rank (LTR) method~\cite{liu2009learning} based on features of CTR, CVR and other user preference scores (e.g., brand or shop preferences, etc) to rank the items and give the top-$k$ results~\cite{lin2019pareto}.
Furthermore reranking methods~\cite{pei2019personalized,ai2018learning,zhuang2018globally,gong2019exact} which consider local ranking context given initial ranked items from LTR will be applied.

Nowadays almost all the above RS models are serving on cloud servers (based on cloud computing~\cite{hayes2008cloud}) and respond to the paging requests from mobile client when user scrolls on the waterfall flow RS (i.e. in client-and-server framework).
So response-time (RT) is a critical metric that affects user experience.
Queries-per-second (QPS) is a factor affecting RT,
which causes computing overhead for serving such complex RS models on cloud servers.
So that we cannot make the paging size much smaller, which prevents the adjustment of recommendation results in time.
Network bandwidth and latency are other factors affecting user experience in RS.
Almost all the models in both matching and ranking stages depend on user behaviors (i.e. user interaction with items) as input features to ensure the personalization.
And user behaviors are collected on mobile client and sent to cloud servers over the network,
in which network bandwidth and latency may limit the amount and timeliness of user behaviors.
To summarize, RS based only on cloud computing does not work perfectly in waterfall flow scenario.
%as communication overhead makes it delayed for both user behavior modeling and system feedback.

%\subsection{Reranking Algorithms}
%\label{sec:reranking_related}
%XXXX
%In the last few decades, cloud computing~\cite{hayes2008cloud} has achieved remarkable development.
%At the same time, it also faces some problems in the following: 
%\begin{itemize}
%\item 
%Explosive growth of internet applications and users brings the pressure of cloud storage.
%\item 
%The deployment of large-scale neural networks in online systems creates tremendous pressure on cloud computing.
%\item 
%For some applications with high real-time requirements, the huge communication overhead with the cloud system is also the bottleneck for interaction and experience.
%\item 
%The centralized computing model on cloud also brings operation and maintenance costs and failure risks.
%\item 
%The issue of data privacy is getting more and more attention.
%\end{itemize}
%Nowadays almost all works of RS in terms of both systems and algorithms are based on cloud computing.

%Edge computing is a buzzword now~\footnote{\url{https://www.theverge.com/circuitbreaker/2018/5/7/17327584/edge-computing-cloud-google-microsoft-apple-amazon}}. 
%%It has the potential to address the concerns of response time
%%requirement, network bandwidth constraint, as well as data safety and privacy~\cite{shi2016edge}.
%It is ideal for applications that require high real-time performance, e.g., smart home~\cite{vallati2016mobile}, smart city~\cite{taleb2017mobile} and RS on mobile (here mobile device is the edge).
%But unfortunately, no previous work has discussed the application of edge computing to RS in terms of systems and algorithms.
%Furthermore by applying edge computing,
%RS can utilize users' more plentiful and detailed behaviors on device without considering network bandwidth limitations and alleviate the problem of data privacy.

%\cite{guo2019buying,hard2018federated} to be done.
